Bernoulli Factories and Black-Box Reductions in Mechanism Design

We provide a polynomial time reduction from Bayesian incentive compatible mechanism design to Bayesian algorithm design for welfare maximization problems. Unlike prior results, our reduction achieves exact incentive compatibility for problems with multi-dimensional and continuous type spaces. The key technical barrier preventing exact incentive compatibility in prior black-box reductions is that repairing violations of incentive constraints requires understanding the distribution of the mechanism's output, which is typically #P-hard to compute. Reductions that instead estimate the output distribution by sampling inevitably suffer from sampling error, which typically precludes exact incentive compatibility. We overcome this barrier by employing and generalizing the computational model in the literature on $\textit{Bernoulli factories}$. In a Bernoulli factory problem, one is given a function mapping the bias of an "input coin" to that of an "output coin", and the challenge is to efficiently simulate the output coin given only sample access to the input coin. This is the key ingredient in designing an incentive compatible mechanism for bipartite matching, which can be used to make the approximately incentive compatible reduction of Hartline et al. (2015) exactly incentive compatible.

==> combinatorial.tex <==
\newcommand{\ground}{\mathcal{G}}
\newcommand{\ber}[1]{\textrm{Ber}(#1)}
\section{Combinatorial Bernoulli Factories and Applications}
In Section~\ref{sec:single} we discussed the \emph{Bernoulli race}, which formally speaking is the following problem.

\begin{definition}[\textbf{Bernoulli Race Problem}]
 Suppose $\ground$ is a ground set of $n$ elements. Given access to sampling oracles $B_i~\sim\ber{q_i}$ for $i\in\ground$ with means $\qbf\in\Delta_{n}$, output a distribution 
\end{definition}

\subsection{Basic Definitions}
\subsection{2-Uniform Matroid Bernoulli Factory}
\subsection{Extension to k-uniform Matroid and Perfect Matching}
\subsection{Applications in Mechanism Design}

==> gamma.tex <==
\paragraph{Estimating $\mathbf{\gamma}$ through sampling.}
We need to initialize $\gamma$ such that $\frac{\opt}{k}\leq\gamma\leq O(1)\cdot\frac{\opt}{k}$. To this end, we find the empirical estimate $\hat{\vbf}_i$ of $\vbf_i$ for all $i\neq i^*$ by sampling (Recall that $i^*$ denotes the index of the real agent replica, i.e.~the replica that corresponds to the real agent's reported type). We then use those estimates  to solve the following convex program, denoted by \emph{empirical} RSLM.
\begin{equation*}
\begin{array}{rrclcl}
\displaystyle \underset{\{\xbf_i\}_{i\neq i^*}}{\text{maximize}} & \multicolumn{3}{l}{\sum_{i\neq i^*}\xbf_i \cdot \hat\vbf_i+\delta\sum_{i\neq i^*}H(\xbf_i)} \\
\textrm{s.t.} & \xbf_{i} & \in &\Delta_m & & i\in[mk]\setminus i^* \\
&\displaystyle \sum_{i\neq i^*}x_{i,j} & \leq & k & & j=1,\ldots,m \\
\end{array}
\end{equation*}
First of all, as we never ask the real agent for its type, this step is obviously incentive compatible. Moreover, suppose $\xbf^*$ is the optimal solution of the empirical RSLM convex program and $\xbf^{**}$ is the optimal solution of the original RSLM convex program. Suppose $\forall (i,j): \hat{v}_{i,j}\geq v_{i,j}-\epsilon$ for some $\epsilon >0$ (This event holds with high probability with enough samples). As $\{\xbf_i^{**}\}_{i\neq i^*}$ also forms a feasible solution for the empirical RSLM, we have:
\begin{align}
\frac{\texttt{OPT}}{k}\geq \frac{\texttt{OPT}_{\textrm{empirical}}}{k}\triangleq& \frac1k \left(\sum_{i\neq i^*}\xbf^*_i \cdot \hat\vbf_i+\delta\sum_{i\neq i^*}H(\xbf^*_i)\right)\geq  \frac1k \left(\sum_{i\neq i^*}\xbf^{**}_i \cdot \hat\vbf_i+\delta\sum_{i\neq i^*}H(\xbf^{**}_i)\right)\nonumber\\
\geq & \frac1k \left(\sum_{i}\xbf^{**}_i \cdot \hat\vbf_i+\delta\sum_{i}H(\xbf^{**}_i)-(1+\delta\log(m))\right)\nonumber\\
\geq& \frac1k \left(\sum_{i}\xbf^{**}_i \cdot \vbf_i+\delta\sum_{i}H(\xbf^{**}_i)-(\epsilon\cdot km+1+\delta\cdot\log(m))\right)\nonumber\\
=&\label{eq:gamma}
 \frac{\texttt{OPT}}{k}-\epsilon\cdot m-\frac{1}{k}-\frac{\delta\cdot\log(m)}{k}\overset{}{\geq}\frac{\texttt{OPT}}{k}\left(1-\frac{\epsilon}{\delta\cdot\log(m)}-\frac{1}{\delta\cdot mk\log(m)}-\frac{1}{mk}\right)
\end{align}
where the last inequality holds as $\texttt{OPT}$ is bounded below by the value of the uniform allocation, i.e. $\texttt{OPT}\geq \delta\cdot mk\log(m)$. Now suppose $\delta\cdot m\log(m)=\Omega(1)$. By setting $\epsilon=O(\delta\cdot\log(m))$, the right hand side will be lower-bounded by $c\cdot\frac{\texttt{OPT}}{k}$ for some constant $c<1$. We now have the following technical lemma.

\begin{lemma} 
\label{lem:gamma}
Given $\eta\in(0,1)$, let $\gamma\triangleq 1/(ck)\cdot \texttt{OPT}_{\textrm{empirical}}$, where each $\hat{v}_{i,j}$ is the empirical mean of $L$ samples. If $\delta\cdot m\log(m)=\Omega(1)$ and $L=\Omega\left(\frac{\log(\frac{m^2k}{\eta})}{\delta^2\cdot \log^2(m)}\right)$, then with probability at least $1-O(\eta)$ we have $\frac{\opt}{k}\leq\gamma\leq O(1)\cdot\frac{\opt}{k}$.
\end{lemma}  
\begin{proof}
By using the Chernoff-Hoeffding inequality, with probability at least $1-O(\eta)$ we have $\forall (i,j): \hat{v}_{i,j}\geq v_{i,j}-O(\delta\cdot\log(m))$  when $L=\Omega\left(\frac{\log(\frac{m^2k}{\eta})}{\delta^2\cdot \log^2(m)}\right)$. The lemma then holds due to (\ref{eq:gamma}).\qed
\end{proof}


==> prelim-md.tex <==

\section{Basics of Mechanism Design}
\label{sec:prelim-md}

\paragraph{Multi-dimensional Bayesian mechanism design.}
Suppose there are $\nBidder$ agents, where agent $k$ has private
\emph{type} $\type{k}$ from \emph{type space} $\typeS{k}$. The
\emph{type profile} of all agents is denoted by
$\typeP=(\type{1},\ldots,\type{n})\in \typeS{1}\times\ldots\times
\typeS{n}$. Moreover, we assume types are drawn independently from
known prior distributions. For agent $k$, let $\prior{k}$ be the
distribution of $\type{k}\in\typeS{k}$ and
$\priorJ=\prior{1}\times\ldots\times\prior{n}$ be the joint
distribution of types. Suppose there is an \emph{outcome space}
denoted by $\outS$. Agent $k$ with type $\type{k}$ has valuation
$v(\type{k},o)$ for outcome $o\in \outS$, where
$v:(\typeS{1}\cup\ldots\cup\typeS{n})\times \outS\rightarrow [0,1]$ is
a fixed function. Note that we assume agent values are non-negative
and bounded, and w.l.o.g in $[0,1]$.  Finally, we allow charging
agents with non-negative money \emph{payments} and we assume agents
are \emph{quasi-linear}, i.e. an agent with private type $t$ has
\emph{utility} $u=v(t,o)-p$ for the outcome-payment pair $(o,p)$.
 
\paragraph{Algorithms, mechanisms, and interim allocation rules.}
An \emph{allocation algorithm} $\alloc$ is a mapping from type
profiles $\typeP{}$ to outcome space $\outS$. A (direct revelation)
mechanism $\mech$ is a pair of \emph{allocation rule} and
\emph{payment rule} $(\alloc,\payP)$, in which $\alloc$ is an
allocation algorithm and $\payP=(\pay{1},\ldots,\pay{n})$ where each
$\pay{k}$ (denoted by the payment rule for agent $k$) is a mapping
from type profiles $\typeP$ to $\mathbb{R}_{+}$. In fact, one can
think of the interaction between strategic agents and a mechanism as
following: agents submit their \emph{reported types}
$\bidP=(\bid{1},\ldots,\bid{n})$ and then the mechanism $\mech$ picks
the outcome $o=\alloc(\bidP)$ and charges each agent $k$ with its
payment $\pay{k}(\bidP)$. We also consider \emph{interim allocation
  rule}, which is the allocation from the perspective of one agent
when the other agent's types are drawn from their prior
distribution. More concretely, we abuse notation and define
$\alloc^k(s_k)\triangleq \alloc(s^{k},\typeO{-k})$ to be the
distribution over outcomes induced by $\alloc$ when agent $k$'s type
is $s^{k}$ and other agent types are drawn from
$\priorJ^{-k}$. Similarly, for agent $k$ we define \emph{interim
  payment rule}
$\pay{k}(s^{k})\triangleq\ex{\typeO{-k}\sim\priorJ^{-k}}{\pay{k}(s^{k},\typeO{-k})}$,
and \emph{interim value} $v^k(s^{k})\triangleq
\ex{\typeO{-k}\sim\priorJ^{-k}}{v(s^{k},\alloc^k(s^{k},\typeO{-k}))}$. In
most parts of this paper, we focus only on one agent, e.g. agent $k$,
and we just work with the interim allocation algorithm
$\alloc^{k}(.)$. When it is clear from the context, we drop the
agent's superscript, and therefore $\alloc(s)$ denotes the
distribution over outcomes induced by $\alloc(s,\typeO{-k})$ when
$\typeO{-k}\sim \priorJ^{-k}$.

We also use standard incentive compatibility notions, i.e. BIC and
DSIC. In this paper, we focus on the expected welfare objective. For
more details, see Appendix~\ref{Appendix:mechnotations}.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> single-agent-pre-shaddin-pass.tex <==
\newcommand{\Di}[1]{\mathcal{D}_{#1}}
\newcommand{\vmax}{v_{\textrm{max}}}
%\newcommand{\vbf}{\mathbf{v}}
\newcommand{\qbf}{\mathbf{q}}
\section{Single-Agent Multiple-Urns Problem}
\label{sec:single}
Consider the following basic mechanism design problem for only one agent. Suppose we have $n$ urns, where each urn $i$ has an associated probability distribution $\Di{i}$ over outcomes in  $\outS$. Given the reported type of the agent, the mechanism designer wants to assign one of the urns to her and charge her with some payment, such that (1) the agent bests off by truthful reporting her type (2)her welfare is close to the optimal one. However, the designer \emph{does not} know the distributions $\{\mathcal{D}_i\}$ and can only get samples from those. 
\paragraph{Question:} \emph{Can we design a truthful near-optimal welfare mechanism only with polynomial number of samples to sampling devices?}

In Section~\ref{sec:single-defining} we first formally define the above mentioned problem. We then discuss a related algorithmic problem which we call \emph{Bernoulli race}. In the Bernoulli race problem, the objective is to design an algorithm for picking one of many unknown coins by only tossing them, such that the marginal probability of each coin being picked will be proportional to its bias. We then show how this algorithmic tool will be applied to truthful mechanism design for the single agent multiple urns problem and introduce the \emph{logistic Bernoulli race}. We finally propose a polynomial sample complexity algorithm by combining all the pieces.


\subsection{Problem Definition}
\label{sec:single-defining}
%Suppose we have $n$ urns, where urn $i$ has the probability distribution $\mathcal{D}_i$ over outcomes in the set $\mathcal{O}$ (this set can be either a discrete or a continuous set). Consider an agent with a type space $\mathcal{T}$ and a value function $\textrm{Val}:\mathcal{T}\times\mathcal{O}\rightarrow [0,1]$ that maps agent's private type and the picked outcome into a value in $[0,1]$. For $t\in\tau$, let $V_i(t)\triangleq\mathbb{E}_{O\sim \mathcal{D}_i}\{\textrm{Val}(t,O)\}$ and $V_{\textit{max}}(t)=\underset{i\in[n]}{\max}~V_i(t)$. In a direct mechanism design setting, an agent submits his reported type $t$ and a mechanism maps $\mathbf{V}=[V_1(t),\ldots,V_n(t)]$ to an allocation $\mathbf{q}(\mathbf{V})$ and a non-negative payment $p(\mathbf{V})$, where allocation $\mathbf{q}\in \Delta ^n$ is a distribution over urns $1,\ldots,n$. The goal is to design a Dominant Strategy Incentive Compatible (DSIC) mechanism, which its welfare approximates optimal welfare $V_{\textit{max}}(t)$ with an additive loss of at most $\epsilon$. Moreover, we are interested in mechanisms for which  the allocation and payment can be implemented with $\textrm{poly}(n,\frac{1}{\epsilon})$ number of sample queries to an oracle that generates a random sample $\textrm{Val}(t,O)$, for some $t\in \tau$ and $O\sim D_i$. 

 Suppose we have $m$ urns indexed by numbers $[1:m]$. Consider an agent with the type space $\typeS{}$ and value function $v:\mathcal{T}\times\mathcal{O}\rightarrow [0,1]$ as in Section~\ref{sec:prelim}. For $t\in\tau$, let $v_i(t)\triangleq\ex{O\sim \mathcal{D}_i}{v(t,O)}$ and $\vmax(t)={\max}_{i\in[m]}~v_i(t)$.  A direct mechanism first elicits agent's reported type $t$ and then maps $t$ to a distribution $\mathbf{q}$ over urns, called the \emph{allocation},  and a non-negative \emph{payment} $p$. The goal is to design a (randomized) DSIC mechanism with at most $\epsilon$ welfare-loss compared to the optimal welfare $\vmax(t)$ in expectation. Moreover, we are interested in mechanisms for which  the allocation and the payment can be implemented with $\textrm{poly}(m,\frac{1}{\epsilon})$ sample queries to the oracle that given a fixed $t$ and index $i\in[m]$, generates a fresh sample $v(t,o)$ where $o\sim \Di{i}$. 
 
\begin{remark}
Let $\vbf=[v_1(t),\ldots,v_m(t)]$. For brevity,  we sometimes abuse the notation and use $\qbf(\vbf)$ and $p(\vbf)$ to refer to the allocation and the payment respectively. Also, for simplicity, we drop the agent type $t$ when it is clear from the context.
\end{remark}
\subsection{Bernoulli Race}
As the first step to find an allocation algorithm for the single agent multiple-urns problem, we look at the following puzzle, which can be thought of as a \emph{combinatorial Bernoulli factory} problem. 

\begin{definition}[\textbf{Bernoulli Race}]
\label{def:ber-race}
 Given sample access to Bernoulli random variables with unknown biases $\vbf=[v_1,\ldots,v_m]$, output a distribution over $[m]$ with marginals $\qbf$, where
$$\displaystyle{i\in[m]:~~q_i=\frac{v_i}{\displaystyle\sum_{j\in [m]}v_j} }$$
\end{definition} 
Here we propose two algorithms for solving this problem, where each one uses a different approach and techniques. While the first algorithm is simpler, it is indeed slower than the second one.

\begin{algorithm}[ht]
\small
\algblock[Name]{Start}{End}
\algblockdefx[NAME]{START}{END}%
[2][Unknown]{Start #1(#2)}%
{Ending}
\algblockdefx[NAME]{}{OTHEREND}%
[1]{Until (#1)}
 \caption{ (for Bernoulli Race)
     \label{alg:ber-race2}}
      \begin{algorithmic}[1]
        \State{\textbf{input}}~ sample access to $m$ coins with biases $v_1,\ldots,v_m$.
        \For {$i=1~\textrm{to}~n$}
        \Repeat
        \State Draw fresh a sample $x\sim\textrm{exp(1)}$ and let $x_i\leftarrow x_i+x$.
        \State Flip coin $i$.  
        \Until{coin flip outcome $=``1"$}
        \EndFor
        \State {\textbf{output:}  $\argmin{j\in[m]}{x_j}$}.
      \end{algorithmic}
\end{algorithm}
\begin{lemma}
Algorithm~\ref{alg:ber-race2} uses $\sum_{i\in[m]}\frac{1}{v_i}$ sample queries in expectation before termination, and it outputs the Bernoulli race distribution as in Definition~\ref{def:ber-race}.
\end{lemma}
\begin{proof}
In order to prove,  we use basic facts about exponential random variables. In particular, we use the following facts:
\begin{itemize}
\item[1.] Sum of $k$ independent $\textrm{exp}(\lambda)$ variables when $k\sim \textrm{geometric}(v)$ is a $\textrm{exp}(\lambda/ v)$ variable.  
\item[2.] Given independent $x_j\sim\textrm{exp}(\lambda_i)$ variables, $x_i$ is the smallest with probability $\frac{\lambda_i^{-1}}{\sum_{i}\lambda_j^{-1}}$.
\end{itemize}
Now, note that each $x_i$ is sum of $k_i$ independent $\textrm{exp}(1)$ variables, where $k_i$ is the number of coin $i$ flips until the first $1$. Therefore, $k_i$ is a $\textrm{geometry}(v_i)$ random variable and so $x_i\sim\textrm{exp}(1/v_i)$ based on the first fact above. Moreover, $\ex{}{k_i}=1/v_i$, and therefore the algorithm terminates with $\sum_{i\in[m]}1/v_i$ coin tosses in expectation. Using the second fact above,
\begin{equation}
\Pr\{i=\argmin{j\in[m]}{x_j}\}=\frac{v_i}{\displaystyle\sum_{j\in[m]}v_{j}}.
\end{equation}
\qed
\end{proof}
\begin{algorithm}[ht]
\small
\algblock[Name]{Start}{End}
\algblockdefx[NAME]{START}{END}%
[2][Unknown]{Start #1(#2)}%
{Ending}
\algblockdefx[NAME]{}{OTHEREND}%
[1]{Until (#1)}
 \caption{ (for Bernoulli Race)
     \label{alg:ber-race1}}
      \begin{algorithmic}[1]
        \State{\textbf{input}}~ sample access to $m$ coins with biases $v_1,\ldots,v_m$.
        \State{\textbf{initialize}}~$\textrm{success}=\texttt{FALSE}$.
        \Repeat
        \State Pick coin $i^*\in[1:n]$ uniformly at random and flip it. 
        \If {$\textrm{coin flip outcome}=``1"$}
        \State $\textrm{winner}\leftarrow i^*$.
        \State $\textrm{success}\leftarrow \texttt{TRUE}$.
        \EndIf
        \Until {$\textrm{success}=\texttt{TRUE}$}
        \State {\textbf{output:} $\textrm{winner}$}
      \end{algorithmic}
\end{algorithm}
\begin{lemma}
\label{lemma:ber-race-dist}
Algorithm~\ref{alg:ber-race1} uses $\frac{m}{\sum_{i\in[m]}v_i}$ sample queries in expectation before termination, and it outputs the Bernoulli race distribution as in Definition~\ref{def:ber-race}.
\end{lemma}
\begin{proof}
At each iteration, the algorithm terminates if the flipped coin outputs $1$ and iterates otherwise.  So, at each iteration $k\in\mathbb{N}$ the algorithm terminates with probability $\frac{1}{m}\sum_{i\in[m]}v_i$, conditioned on not being terminated before this time. Therefore one can look at the total number of iterations of the algorithm as a geometric random variable with parameter $\frac{\sum_{i\in [m]}v_i}{m}$, and so we have:
\begin{equation}
\ex{}{\textrm{number of sample queries}}=\ex{}{\textrm{number of iterations before termination}}=\frac{m}{\sum_{i\in [m]}v_i}.
\end{equation}
Moreover, the output distribution is the following.
\begin{align*}
\textrm{Pr}\{\textrm{winner}=i\}&=\sum_{k\in \mathbb{N}}\textrm{Pr}\{(\textrm{winner}=i)~\& ~\textrm{Algorithm~\ref{alg:ber-race1} does not terminate before $k$}\}\nonumber\\
&=\frac{v_i}{m}\sum_{k\in \mathbb N}\left (1-\frac{1}{m}\sum_{j\in[m]}v_j\right)^k=\frac{\frac{v_i}{m}}{\frac{1}{m}\displaystyle\sum_{j\in [m]}v_j}.
\end{align*}\qed
\end{proof}
\subsection{On The Road To Truthfulness: Logistic Bernoulli Race}
A well-studied approach to design dominant strategy truthful allocations is using a class of allocations called \emph{affine maximizers}. 
\begin{definition}
Given the agent's reported type $t$, an allocation is an \emph{affine maximizer} if there exists a constant $\alpha>0$, a function $\beta:\Delta_m\rightarrow  \mathbb{R}$ and a range $\mathcal{X}\subseteq \Delta_m$ such that the allocation selects a distribution $\qbf^*\in \mathcal{X}$ over urns that maximizes $\alpha\qbf.\vbf(t)+\beta(\qbf)$.
\end{definition}
The following theorem~\citep{lavi2003towards,dobzinski2009power} establishes the truthfulness of  affine maximizers.
\begin{theorem}[\citet{lavi2003towards,dobzinski2009power}, Interpreted] Let allocation $\alloc$ be an affine maximizer. There are payments $\mathbf{p}$ such that $\mathcal{M}=(\alloc,\mathbf{p})$ is a DSIC mechanism.
\end{theorem}
Now, our approach is finding an affine maximizer that (1) it does not suffer from more than $\epsilon$ welfare-loss from optimal welfare, and (2) it is implementable \emph{exactly} by only sampling from urns. In particular, we are interested in a solution that uses Bernoulli race as a black-box. In order to achieve these objectives simultaneously, we consider the standard \emph{entropy regularization} of the welfare objective function. Formally speaking, we consider the following affine maximizer.
\begin{equation}
\label{eq:affine1}
\argmax{\qbf\in\Delta_m} ~~~~\qbf.\vbf +\frac{\epsilon}{\log(m)} H(\mathbf{q}),
\end{equation}
where $H(.)$ is the Shannon's entropy function. This convex program is interesting from two aspects. First, the welfare-loss of its optimal solution is no greater than  $\epsilon$ as $H(\qbf)\leq \log(m)$.  Second, it is easy to show that the following is the unique optimal solution of the convex program in (\ref{eq:affine1}).
\begin{equation}
\label{eq:dist1}
\forall i\in [m]:~~~q^*_i(\vbf)=\frac{e^{\frac{v_i}{\epsilon'}}}{\displaystyle\sum_{j\in[m]}{e^{\frac{v_j}{\epsilon'}}}}
\end{equation}
where $\epsilon'=\frac{\epsilon}{\log m}$. Interestingly,  we show how by sample queries to $\{v(t,o)|o\sim\Di{i}, i\in[m]\}$, one can implement the DSIC allocation rule in (\ref{eq:dist1}). 

\shadowbox{

\begin{minipage}{40em}
\vspace{2mm}
\textbf{DSIC allocation for single-agent multiple-urns problem with sampling.}
\begin{enumerate}
\item For each urn $i$ and given the reported type $t$, generate a  random coin $B_i\sim \textrm{Bern}(v_i)$, where a fresh sample of this coin is generated through the following procedure:
      	\begin{itemize}
      	\item Draw $u_i\sim \textrm{unif}~[0,1]$ independently for each urn. 
      	\item Draw $v(t,o_i)$ independently for each urn, where $o_i\sim \Di{i}$.
      	\item If $u_i\leq v(t,o_i)$, let $B_i=1$. Otherwise, let $B_i=0$.
      	\end{itemize}
\item Given access to the $m$ coins with biases $v_1,\ldots,v_m$, run an algorithm for the \emph{logistic Bernoulli race} defined below to output an urn, and will assign this urn to the agent.
\end{enumerate}
\vspace{1mm}
\end{minipage}
}

\begin{definition}[\textbf{Logistic Bernoulli Race}] 
\label{defn:log-ber-race}
Given sample access to Bernoulli random variables with unknown biases $\vbf=[v_1,\ldots,v_m]$, output a distribution over $[m]$ with marginals $\qbf$, where
\begin{equation}
\forall i\in [m]:~~~q_i= \frac{e^{\frac{v_i}{\epsilon'}}}{\displaystyle\sum_{j\in[m]}{e^{\frac{v_j}{\epsilon'}}}}
\end{equation}
\end{definition}

\begin{algorithm}[ht]
\small
\algblock[Name]{Start}{End}
\algblockdefx[NAME]{START}{END}%
[2][Unknown]{Start #1(#2)}%
{Ending}
\algblockdefx[NAME]{}{OTHEREND}%
[1]{Until (#1)}
 \caption{ Non-Polynomial Logistic Bernoulli Race
     \label{alg:ber-lograce-nonpoly}}
      \begin{algorithmic}[1]
        \State{\textbf{input}}~ sample access to $m$ coins with biases $v_1,\ldots,v_m$.
        \State{\textbf{pre-processing}}~ $\forall i\in[m]$, generate a new coin with bias $\tilde{v}_i=e^{\frac{v_i-1}{\epsilon'}}$ using the following Bernoulli factory:
        \begin{itemize}
        \item Sample $k_i\sim \textrm{Poisson}(\frac{1}{\epsilon'}).$
        \item Flip the $i^{\textrm{th}}$ coin  $k_i$ number of times.
        \item If all the coin flips where $``1"$ output $``1"$, otherwise output $``0"$.
        \end{itemize} 
        \State Run Algorithm~\ref{alg:ber-race1} for new coins $\textrm{Bern($\tilde{v}_i$)}$.
      \end{algorithmic}
\end{algorithm}


\begin{lemma}
\label{lemma:log-ber-race-dist}
Algorithm~\ref{alg:ber-lograce-nonpoly} uses $\frac{m}{\sum_{i\in[m]}m^{\frac{v_i-1}{\epsilon}}}$ sample queries in expectation before termination, and outputs the logistic Bernoulli race distribution as in Definition~\ref{defn:log-ber-race}.
\end{lemma}
\begin{proof}
Due to Lemma~\ref{lemma:ber-race-dist},  Algorithm~\ref{alg:ber-race1} returns a Bernoulli race distribution for biases $\tilde{v}_i$ with the desired sample complexity. Therefore, we only need to show $\tilde{v}_i=e^{\frac{v_i-1}{\epsilon'}}$. Let $B_i$ be the original coin and $\tilde{B}_i$ be the new coin. As $k_i\sim \textrm{Poisson}(\frac{1}{\epsilon'})$ , we have
\begin{align}
\tilde{v}_i=\textrm{Pr}\{\tilde{B}_i=1\}&=\mathbb{E}\left\{\mathbf{1}\{\textrm{all $k_i$ coins-tosses yield $1$}\}\right\}=\mathbb{E}_{k_i}\{\mathbb{E}\{\textrm{all $k_i$ coins-tosses yield $1$}|k_i\}\}\nonumber\\
&=\mathbb{E}_{k_i}\left\{(\mathbb{E}\{{B}_i\})^{k_i}\right\}
=e^{-\frac{1}{\epsilon'}}\sum_{k\in \mathbb{N}}v_i^k\frac{(\frac{1}{\epsilon'})^k}{k!}=e^{\frac{v_i-1}{\epsilon'}}.
\end{align} \qed
\end{proof}

Unfortunately, Algorithm~\ref{alg:ber-lograce-nonpoly} \emph{does not} guarantee the polynomial sample complexity, as promised. In fact, using Lemma~\ref{alg:ber-race1}, the expected number of queries to the sampling oracle is $m/{\sum_{j\in m}e^{\frac{\log(m)(v_j-1)}{\epsilon}}}$, and when $\vmax\leq 1-c$ for a constant $c$ this indeed is exponential in $1/\epsilon$. In the next section, we show how by \emph{truthfully transforming} the values one can ensure $\vmax\approx 1$, and therefore enjoys the polynomial sample complexity.


\subsection{Towards Polynomial Sample Complexity: Levering Step }
\label{sec:levering}
An interesting observation is the following. If we shift the expected values $v_i$ all by the same $\lambda\in\mathbb{R}$, then the allocation probabilities in (\ref{eq:dist1}) \emph{do not} change. Therefore, shifting values, no matter how, is a truthful transformation when combined with the logistic Bernoulli race. This observation leads us to the following question: \emph{can we shift the values  by only sampling, such that $\vmax$ will become close to $1$?}. Surprisingly, the answer is positive. In fact this transformation, which we call \emph{levering step}, can only be done by taking polynomial number of samples from the value oracle. Note that as the final allocation rule is invariant with the choice of $\lambda$, one can use the values themselves to find an appropriate shift.

 Before proceeding further, we modify the affine maximzer in (\ref{eq:affine1}) to get the following program:
\begin{equation}
\label{eq:affine}
\argmax{\qbf\in\Delta_m}{~~~~(1-\frac{\epsilon}{2})~\vbf.\qbf +\frac{\epsilon}{2\log(m)} H(\mathbf{q})}
\end{equation}
Let $\epsilon'\triangleq\frac{\epsilon}{2\log(m)}$ and $v'_i\triangleq(1-\frac{\epsilon}{2})v_i$. Also, let $\vmax'=(1-\frac{\epsilon}{2})\vmax$. As before, the optimal solution $\qbf^*$ forms a DSIC allocation while enjoys a welfare-loss bounded by $\epsilon$, simply because
 \begin{equation}
 (1-\frac{\epsilon}{2})\vmax\leq (1-\frac{\epsilon}{2}) \sum_{i=1}^m q^*_iv_i+\epsilon' H(\mathbf{q}^*)\leq (1-\frac{\epsilon}{2})\sum_{i=1}^m q^*_iv_i+\frac{\epsilon}{2}
 \end{equation}
 which shows $\sum_{i=1}^m q^*_iv_i\geq \vmax-\frac{\frac{\epsilon}{2}}{1-\frac{\epsilon}{2}}\geq  \vmax-\epsilon$. Lets also recap the linear multivariate Bernoulli factory result due to \citet{Huber2015OptimalLB} in Theorem~\ref{thm:huber}. We use this mixing algorithm for our levering.
  
Now, informally speaking, we do the following to lever the values. For each coin $i$, we take many samples from all coins to have an unbiased estimation of $\vmax$, denoted by $\hat{v}_{\textrm{max}}$. We then generate a coin with bias $\approx 1-\ex{}{\hat{v}_{\textrm{max}}}$ and mix that coin with our original coin using Theorem~\ref{thm:huber} to lever up the bias. Performing this step for each coin will ensure there exists at least one coin whose bias is close to $1$, and therefore the logistic Bernoulli race algorithm, i.e. Algorithm~\ref{alg:ber-lograce-nonpoly},  converges in polynomial many iterations. Formally speaking, we have the the following levering procedure.
  \floatname{algorithm}{Procedure}
\begin{algorithm}[ht]
\small
\algblock[Name]{Start}{End}
\algblockdefx[NAME]{START}{END}%
[2][Unknown]{Start #1(#2)}%
{Ending}
\algblockdefx[NAME]{}{OTHEREND}%
[1]{Until (#1)}
 \caption{ Levering Step
     \label{alg:levering}}
      \begin{algorithmic}[1]
      	\State \textbf{input:} sample access to  $m$ coins $\{B_i\}_{i=1}^m$, where $\mathbb{E}\{B_i\}=v_i$.
      	\State \textbf{output:} sample access to $m$ coins $\{\tilde{B}_i\}_{i=1}^m$.

		\State Generate a $B'_i\sim \textrm{Bern}((1-\frac{\epsilon}{2})v_i)$ random coin as following:
		\begin{itemize}
		
		 
		\item  Draw an independent sample $u\sim\textrm{unif}[0,1]$.
		\item  Draw an independent  sample $B_i$ from sampling oracle $i$.
		\item  If $u\leq (1-\frac{\epsilon}{2})$ and $B_i=1$, then $B'_i=1$. Otherwise, $B'_i=0$.
		\end{itemize}  
		\State Generate a $Z_i$ random coin as following:
	\begin{itemize}
	
	
		
		\item Draw an independent sample $u\sim \textrm{unif}~[0,1]$. 
		\item Draw an independent sample from random variable $\lambda$ by:
		\begin{itemize}
		
      	\item For each $l$, draw $K\triangleq\lceil\frac{144m}{\epsilon^3}\rceil$ i.i.d samples from $B'_l$, denoted by $\{B'_{l,j}\}_{j=1}^{K}$.
      	\item For each $l$, let $\hat{v}_l\triangleq \frac{1}{K}\sum_{j=1}^{K}B'_{l,j}$.
      	\item Define $\hat{v}_{\textrm{max}}\triangleq\underset{l\in[1:m]}{\max} \hat{v}_l$.
      	\item Let $\lambda=\max(1-\hat{v}_{\textrm{max}}-\frac{3\epsilon}{4},0)$. 
		\end{itemize}
		\item If $u\leq \lambda$, then $Z_i=1$. Otherwise, let $Z_i=0$.
       \end{itemize}
        \State Given access to coins $B'_i$ and $Z_i$, use the algorithm in Theorem~\ref{thm:huber} to generate the coin $\tilde{B}_i$ with mean $\mathbb{E}\{B'_i\}+\mathbb{E}\{Z_i\}=(1-\frac{\epsilon}{2})v_i+\mathbb{E}\{\lambda\}$. 
\end{algorithmic}
\end{algorithm}
  
  
  
  
  
  
  
  
  
  
  
  
  
%\begin{algorithm}[ht]
%\small
%\algblock[Name]{Start}{End}
%\algblockdefx[NAME]{START}{END}%
%[2][Unknown]{Start #1(#2)}%
%{Ending}
%\algblockdefx[NAME]{}{OTHEREND}%
%[1]{Until (#1)}
% \caption{ Truthful Pre-Processing
%     \label{alg:logisticrace}}
%      \begin{algorithmic}[1]
%      	\State \textbf{input:} access to Bernoulli sampling oracles $\{B_i\}_{i=1}^n$, where $\mathbb{E}\{B_i\}=V_i$.
%%      	\State Generate a random source that outputs samples $\hat{V}_{\textit{max}}$ by:
%%      	\begin{itemize}
%%      	\item For each $i$, draw $K\triangleq\lceil\frac{8n}{\epsilon^3}\rceil$ i.i.d samples from $B_i$, denoted by $\{B_i^{(j)}\}_{j=1}^{K}$.
%%      	\item  For each $i$, let $\hat{V}_i\triangleq \frac{1}{K}\sum_{j=1}^{K}B_i^{(j)}$.
%%      	\item Let $\hat{V}_{\textit{max}}=\underset{i\in[1:n]}{\max} \hat{V}_i$. 
%%      	\end{itemize}
%%      	\State Define a random source $\lambda\triangleq\max(1-\hat{V}_{\textit{max}}-\frac{3\epsilon}{4},0)$. 
%%      	\State For each urn $i$, generate a random coin $\tilde{B}_i\sim \textrm{Bern}(V'_i+\mathbb{E}(\lambda))$ by:
%%      	\begin{itemize}
%%      	\item Generate a $Z_i\sim \textrm{Bern}(\mathbb{E}(\lambda))$ random coin as following:
%%		\begin{itemize}
%%		\item Draw $G_i\sim \textrm{Unif}~[0,1]$ independently for each urn. 
%%		\item Draw a fresh sample from $\lambda$.
%%		\item If $G_i\leq \lambda$, let $G_i=1$. Otherwise, let $G_i=0$.
%%        \end{itemize}	
%%        \item Given access to coins $B_i$ and $Z_i$, use the algorithm in Theorem~\ref{thm:huber} to generate the coin $\tilde{B}_i$ with mean $\mathbb{E}\{B_i\}+\mathbb{E}\{Z_i\}=V'_i+\mathbb{E}\{\lambda\}$. 
%%         \end{itemize}
%        \State $\textrm{success} =\textrm{FALSE}$
%		\Repeat
%		\State Sample $i$ from $1,2,\ldots,n$ uniformly at random.
%		\State Sample integer $m$ from $\textrm{Poisson}(\frac{1}{\epsilon'})$.
%		\State Toss $m$ independent coins from sampling oracle  $\tilde{B}_i\sim \textrm{Bern}(V'_i+\mathbb{E}(\lambda))$, each sample coin generated by: 
%		\Start
%		\State -- Generate a $B'_i\sim \textrm{Bern}(V'_i)$ random coin as following:
%		\Start 
%		\State $\circ$ Draw an independent sample $U\sim\textrm{Unif}[0,1]$.
%		\State $\circ$ Draw an independent  sample $B_i$ from sampling oracle $i$.
%		\State  $\circ$ If $U\leq (1-\frac{\epsilon}{2})$ and $B_i=1$, then $B'_i=1$. Otherwise, $B'_i=0$.
%		\End   
%		\State -- Generate a $Z_i\sim \textrm{Bern}(\mathbb{E}(\lambda))$ random coin as following:
%		\Start
%		
%		\State  $\circ$ Draw an independent sample $U\sim \textrm{Unif}~[0,1]$. 
%		\State  $\circ$ Draw an independent sample from random variable $\lambda$ by:
%		\Start
%      	\State  $\circ$ $\circ$ For each $l$, draw $K\triangleq\lceil\frac{144n}{\epsilon^3}\rceil$ i.i.d samples from $B'_l$, denoted by $\{B'_{l,j}\}_{j=1}^{K}$.
%      	\State   $\circ$ $\circ$ For each $l$, let $\hat{V}_l\triangleq \frac{1}{K}\sum_{j=1}^{K}B'_{l,j}$.
%      	\State  $\circ$ $\circ$ Define $\hat{V}_{\textit{max}}\triangleq\underset{l\in[1:n]}{\max} \hat{V}_l$.
%      	\State  $\circ$ $\circ$ Let $\lambda=\max(1-\hat{V}_{\textit{max}}-\frac{3\epsilon}{4},0)$. 
%		\End
%		\State  $\circ$ If $G\leq \lambda$, then $Z_i=1$. Otherwise, let $Z_i=0$.
%        \End
%        \State -- Given access to coins $B'_i$ and $Z_i$, use the algorithm in Theorem~\ref{thm:huber} to generate the coin $\tilde{B}_i$ with\\
%        
%         $~~~~~~~~~~~$ mean $\mathbb{E}\{B'_i\}+\mathbb{E}\{Z_i\}=V'_i+\mathbb{E}\{\lambda\}$. 
%		\End
%		\If { all $m$ coin-tosses yield $1$ }
%		\State $\textrm{winner}=i$.
%		\State  $\textrm{success} =\textrm{TRUE}$.
%		\EndIf
%		\Until {$\textrm{success} =\textrm{TRUE}.$}   	
%		\State \textbf{output:} winner.
%\end{algorithmic}
%\end{algorithm}

\subsection{Correctness and Polynomial Sampling  Complexity }

Putting all the pieces together, we end up with the following polynomial algorithm for the logistic Bernoulli race problem. 
 \floatname{algorithm}{Algorithm}
\begin{algorithm}[ht]
\small
\algblock[Name]{Start}{End}
\algblockdefx[NAME]{START}{END}%
[2][Unknown]{Start #1(#2)}%
{Ending}
\algblockdefx[NAME]{}{OTHEREND}%
[1]{Until (#1)}
 \caption{ Polynomial Logistic Bernoulli Race
     \label{alg:ber-lograce}}
      \begin{algorithmic}[1]
        \State{\textbf{input}}~ sample access to $m$ coins  $\{B_i\}_{i=1}^m$ with biases $v_1,\ldots,v_m$.
        \State Use Procedure~\ref{alg:levering} to generate sample access to $m$ coins $\{\tilde{B}_i\}_{i=1}^m$.
        \State Run Algorithm~\ref{alg:ber-lograce-nonpoly} for new coins $\{\tilde{B}_i\}_{i=1}^m$ and output the selected coin.
      \end{algorithmic}
\end{algorithm}

In this section, we provide a detailed proof of its polynomial sample complexity. We start by the following crucial lemma, whose proof is provided in Appendix~\ref{app:omitted}. This lemma shows why we can use Theorem~\ref{thm:huber} to implement mixing step (step 5) of Procedure~\ref{alg:levering} with polynomial sample queries, while ensuring the maximum of new biases is close to $1$. 
\begin{lemma}
\label{lemma:bound}
For the Procedure~\ref{alg:levering}, the followings hold:
\begin{itemize}
\item There exists an urn $j$ such that $\mathbb{E}\{\tilde{B}_j\}=v'_j+\mathbb{E}\{\lambda\}\geq 1-\frac{9\epsilon}{8}$.
\item For each urn $i$, $\mathbb{E}\{\tilde{B}_i\}=v'_i+\mathbb{E}\{\lambda\} \leq 1-\frac{\epsilon}{4}$.
\end{itemize}
\end{lemma}
We now have all the necessary ingredient to show correctness and polynomial sample complexity of the Algorithm~\ref{alg:ber-lograce}.
\begin{theorem}
\label{thm:single}
Given access to Bernoulli sampling oracles $\{B_i\}_{i=1}^m$, Algorithm~\ref{alg:ber-lograce} terminates with:
\begin{itemize}
 \item $\textrm{Pr
}\{\textrm{winner}=i\}=q^*_i(\mathbf{v})$, where $\qbf^*$ is the optimal solution of the affine maximization in~(\ref{eq:affine}),
\item $O(\frac{m^{4.125}\log(m)}{\epsilon^5})$ samples queries to the given oracles in expectation.
\end{itemize}
\end{theorem}
\begin{proof}
First of all, by transforming the values from $\vbf$ to $\vbf'$ combined with Lemma~\ref{lemma:log-ber-race-dist}, we have 

$$\textrm{Pr}\{\textrm{winner}=i\}=\frac{e^{\frac{\ex{}{\tilde{B}_i}}{\epsilon'}}}{\sum_{j\in[m]}{e^{\frac{\ex{}{\tilde{B}_j}}{\epsilon'}}}}=\frac{e^{\frac{v'_i}{\epsilon'}}}{\sum_{j\in[m]}{e^{\frac{v'_j}{\epsilon'}}}}$$


where the last equality holds because $\mathbb{E}\{\tilde{B}_i\}=v'_i+\mathbb{E}\{\lambda\}$, for all $i\in [m]$. To prove the sample complexity, first note the following.
\begin{equation}
\mathbb{E}\{\textrm{\# sample queries of Algorithm~\ref{alg:ber-lograce-nonpoly}}\}=\frac{m}{{\sum_{j\in [n]}m^{\frac{\mathbb{E}\{\tilde{B}_j\}-1}{\epsilon}}}}\leq \frac{m}{\underset{j\in [m]}{\textrm{max}}~ m^{\frac{\mathbb{E}\{\tilde{B}_j\}-1}{\epsilon}}}\leq m^{2.125}.
\end{equation}
where the last inequity holds because we know there exists an urn $j$ such that $\mathbb{E}\{\tilde{B}_j\}\geq 1-\frac{9\epsilon}{8}$, due to Lemma~\ref{lemma:bound}. At each iteration of the outer-loop Bernoulli race, the algorithm requires $\frac{1}{\epsilon'}$ sample queries to the oracles $\{\tilde{B}_i\}_{i\in [m]}$. According to Theorem~\ref{thm:huber}, getting a sample from any of $\tilde{B}_i$ requires $\lceil \frac{64}{\epsilon}\rceil$ samples from $B'_i$ and $Z_i$, as for every $i\in [m]$ we have $\mathbb{E}\{B'_i\}+\mathbb{E}\{\lambda\} \leq 1-\frac{\epsilon}{4}$ due to Lemma~\ref{lemma:bound}. Getting a fresh sample from random source $\lambda$ requires $m\lceil \frac{144m}{\epsilon^3}\rceil$ samples from sampling oracles $\{B_j\}_{j\in [m]}$. All in all, this means an iteration of the algorithm only requires $O(\frac{m^2\log (m)}{\epsilon^5})$ samples in expectation, and the algorithm only requires $O(\frac{m^{4.125}\log (m)}{\epsilon^5})$ number of sample queries in expectation before termination.
\end{proof}

